The Spread of Propaganda by Coordinated Communities on Social Media

Large-scale manipulations on social media have two important characteristics: (i) use of propaganda to influence others, and (ii) adoption of coordinated behavior to spread it and to amplify its impact. Despite the connection between them, these two characteristics have so far been considered in isolation. Here we aim to bridge this gap. In particular, we analyze the spread of propaganda and its interplay with coordinated behavior on a large Twitter dataset about the 2019 UK general election. We first propose and evaluate several metrics for measuring the use of propaganda on Twitter. Then, we investigate the use of propaganda by different coordinated communities that participated in the online debate. The combination of the use of propaganda and coordinated behavior allows us to uncover the authenticity and harmfulness of the different communities. Finally, we compare our measures of propaganda and coordination with automation (i.e., bot) scores and Twitter suspensions, revealing interesting trends. From a theoretical viewpoint, we introduce a methodology for analyzing several important dimensions of online behavior that are seldom conjointly considered. From a practical viewpoint, we provide new insights into authentic and inauthentic online activities during the 2019 UK general election.

==> sparklines/sparkline-box-high.tex <==
\begin{sparkline}{1.8}%
    \definecolor{sparkrectanglecolor}{HTML}{525252}
    \sparkrectangle 0 1
\end{sparkline}%

==> sparklines/sparkline-box-low.tex <==
\begin{sparkline}{1.8}%
    \definecolor{sparkrectanglecolor}{HTML}{CCCCCC}
    \sparkrectangle 0 1
\end{sparkline}%

==> sparklines/sparkline-box-med.tex <==
\begin{sparkline}{1.8}%
    \definecolor{sparkrectanglecolor}{HTML}{969696}
    \sparkrectangle 0 1
\end{sparkline}%

==> sparklines/sparkline-box-none.tex <==
\begin{sparkline}{1.8}%
    \definecolor{sparkrectanglecolor}{HTML}{ebebeb}
    \sparkrectangle 0 1
\end{sparkline}%

==> tab-dataset-all.tex <==
\begin{table}[t]
    \begin{minipage}{.5\columnwidth}
        \scriptsize
        \centering
        \adjustbox{max width=1\textwidth}{
        \begin{tabular}{lrrr}
        	\toprule
        	\textbf{hashtag} & \textit{users} & \textit{tweets} \\
        	\midrule
        	\textsf{\#GE2019}	                & 436,356			& 2,640,966			\\
        	\textsf{\#GeneralElection19}	    & 104,616			& 274,095			\\
        	\textsf{\#GeneralElection2019}	    & 240,712			& 783,805			\\
        	\textsf{\#VoteLabour}	            & 201,774			& 917,936			\\
        	\textsf{\#VoteLabour2019}	        & 55,703			& 265,899			\\
        	\textsf{\#ForTheMany}	            & 17,859			& 35,621			\\
        	\textsf{\#ForTheManyNotTheFew}	    & 22,966			& 40,116			\\
        	\textsf{\#ChangeIsComing}	        & 8,170			    & 13,381            \\
        	\textsf{\#RealChange}	            & 78,285			& 274254			\\
        	\textsf{\#VoteConservative}	        & 52,642			& 238,647			\\
        	\textsf{\#VoteConservative2019}	    & 13,513			& 34,195			\\
        	\textsf{\#BackBoris}	            & 36,725			& 157,434			\\
        	\textsf{\#GetBrexitDone}	        & 46,429			& 168,911			\\
        	\midrule
        	\textbf{total}	                    & 668,312			& 4,983,499		        \\
        	\bottomrule
        \end{tabular}}
        \caption{Statistics about data collected via election-specific hashtags.}
        \label{tab:dataset-hashtags}
    \end{minipage}%
    \begin{minipage}{.5\columnwidth}
        \scriptsize
        \centering
        \adjustbox{max width=1\textwidth}{
    	\begin{tabular}{lrrrr}
    		\toprule
    		&&& \multicolumn{2}{c}{\textbf{interactions}}\\
    		\cmidrule{4-5}
    		\textbf{account} & \textit{tweets} && \textit{retweets} & \textit{replies}\\
    		\midrule
    		\textsf{@jeremycorbyn}  & 788   && 1,759,823    & 414,158   \\
    		\textsf{@UKLabour}      & 1,002 && 325,219      & 79,932    \\
    		\textsf{@BorisJohnson}  & 454   && 284,544      & 382,237   \\
    		\textsf{@Conservatives} & 1,398 && 151,913      & 169,736   \\
    		\midrule
    		\textbf{total}          & 3,642	&& 2,521,499    & 1,046,063 \\
    		\bottomrule
    	\end{tabular}}
    	\caption{Statistics about data collected from a few notable accounts.} 
    	\label{tab:dataset-accounts}
    \end{minipage}
\end{table}


==> tab-prop-coord-importance.tex <==
\begin{table*}[t]
    \footnotesize
    \centering
%    \adjustbox{max width=1.3\textwidth}{%
    \centering
    \begin{tabular}{r|p{0.4cm}l|p{0.4cm}l|p{0.4cm}l|p{0.4cm}l|p{0.4cm}l|p{0.4cm}l|p{0.4cm}l|p{0.4cm}l}
        \toprule
         & \multicolumn{2}{c}{overall} & \multicolumn{2}{c}{\texttt{LAB}} & \multicolumn{2}{c}{\texttt{CON}} & \multicolumn{2}{c}{\texttt{TVT}} & \multicolumn{2}{c}{\texttt{SNP}} & \multicolumn{2}{c}{\texttt{ASE}} & \multicolumn{2}{c}{\texttt{B60}} & \multicolumn{2}{c}{\texttt{LCH}} \\
         \midrule
         \multicolumn{17}{l}{\textit{Linear regression model for predicting automation score}} \\ [0.5em]
         propaganda & & \mybar[none]{0.158} & *** & \mybar[high]{0.624} & & \mybar[none]{0.045} & * & \mybar[low]{0.285} & & \mybar[none]{0.376} & & \mybar[none]{0.556} & & \mybar[none]{1.000} & & \mybar[none]{0.306} \\
         coordination & *** & \mybar[high]{1.000} & *** & \mybar[high]{1.000} & ** & \mybar[med]{1.000} & *** & \mybar[high]{1.000} & & \mybar[none]{1.000} & & \mybar[none]{1.000} & & \mybar[none]{0.834} & *** & \mybar[high]{1.000} \\
         \midrule
         \multicolumn{17}{l}{\textit{Logistic regression model for predicting automated users}} \\ [0.5em]
         propaganda & & \mybar[none]{0.033} & * & \mybar[low]{0.346} & & \mybar[none]{0.296} & & \mybar[none]{0.258} & & \mybar[none]{1.000} & & \mybar[none]{0.050} & & \mybar[none]{1.000} & & \mybar[none]{0.073} \\
         coordination & *** & \mybar[high]{1.000} & *** & \mybar[high]{1.000} & & \mybar[none]{1.000} & *** & \mybar[high]{1.000} & & \mybar[none]{0.027} & & \mybar[none]{1.000} & & \mybar[none]{0.810} & & \mybar[none]{1.000} \\
         \midrule
         \multicolumn{17}{l}{\textit{Logistic regression model for predicting suspended users}} \\ [0.5em]
         propaganda & & \mybar[none]{0.080} & & \mybar[none]{1.000} & & \mybar[none]{1.000} & & \mybar[none]{0.929} & & \mybar[none]{0.629} & & \mybar[none]{1.000} & & \mybar[none]{0.194} & & \mybar[none]{1.000} \\
         coordination & & \mybar[none]{1.000} & & \mybar[none]{0.145} & & \mybar[none]{0.817} & & \mybar[none]{1.000} & & \mybar[none]{1.000} & & \mybar[none]{0.463} & & \mybar[none]{1.000} & & \mybar[none]{0.001} \\
         %\midrule
         %n & \multicolumn{2}{c}{10,331} & \multicolumn{2}{c}{5,169} & \multicolumn{2}{c}{2,116} & \multicolumn{2}{c}{2,163} & \multicolumn{2}{c}{439} & \multicolumn{2}{c}{96} & \multicolumn{2}{c}{286} & \multicolumn{2}{c}{62} \\
        \bottomrule
        \multicolumn{17}{p{10cm}}{***, \input{sparklines/sparkline-box-high}: \textit{p} $<$ 0.01 \qquad **, \input{sparklines/sparkline-box-med}: \textit{p} $<$ 0.05 \qquad *, \input{sparklines/sparkline-box-low}: \textit{p} $<$ 0.1 \qquad \input{sparklines/sparkline-box-none}: \textit{p} $\ge$ 0.1}
    \end{tabular}
%    }
    \caption{Feature importance and statistical significance of propaganda and coordination for predicting automation scores, automated users, and suspended users. Results are provided per community as well as for all users.}
\end{table*}


==> unused/tab-corr-prop-vs-automation.tex <==
\begin{table}[t]
    \scriptsize
    \centering
    \begin{tabular}{lcrlcrl}
        \toprule
        \textbf{community} && \multicolumn{2}{c}{$r$} && \multicolumn{2}{c}{$\delta$ (\%)} \\
        \midrule
        \texttt{LAB} && $0.428$ & * && $-0.016$ & ($-6.5\%$) \\
        \texttt{CON} && $-0.688$ & *** && $-0.008$ & ($-3.0\%$) \\
        \texttt{TVT} && $0.836$ & *** && $+0.074$ & ($+26.0\%$) \\
        \texttt{SNP} && $0.358$ &  && $-0.031$ & ($-13.5\%$) \\
        \texttt{B60} && $-0.961$ & *** && $-0.070$ & ($-36.7\%$) \\
        \texttt{ASE} && $0.762$ & *** && $+0.026$ & ($+9.7\%$) \\
        \texttt{LCH} && $0.704$ & *** && $+0.014$ & ($+20.7\%$) \\
        \midrule
        overall && $-0.285$ &  && \multicolumn{2}{c}{--} \\
        \bottomrule
        \multicolumn{7}{l}{***: $p < 0.01$, **: $p < 0.05$, *: $p < 0.1$}
    \end{tabular}
    \caption{\hl{Correlation between propaganda and automation...}\label{tab:corr-prop-vs-automation}}
\end{table}


==> unused/tab-corr-prop-vs-coord.tex <==
\begin{table}[t]
    \scriptsize
    \centering
    \begin{tabular}{lcrlcrl}
        \toprule
        \textbf{community} && \multicolumn{2}{c}{$r$} && \multicolumn{2}{c}{$\delta$ (\%)} \\
        \midrule
        \texttt{LAB} && $-0.193$ &  && $-0.016$ & ($-6.5\%$) \\
        \texttt{CON} && $-0.754$ & *** && $-0.008$ & ($-3.0\%$) \\
        \texttt{TVT} && $0.813$ & *** && $+0.074$ & ($+26.0\%$) \\
        \texttt{SNP} && $-0.404$ & * && $-0.031$ & ($-13.5\%$) \\
        \texttt{B60} && $-0.899$ & *** && $-0.070$ & ($-36.7\%$) \\
        \texttt{ASE} && $0.742$ & *** && $+0.026$ & ($+9.7\%$) \\
        \texttt{LCH} && $0.562$ & *** && $+0.014$ & ($+20.7\%$) \\
        \midrule
        overall && $-0.679$ & *** && \multicolumn{2}{c}{--} \\
        \bottomrule
        \multicolumn{7}{l}{***: $p < 0.01$, **: $p < 0.05$, *: $p < 0.1$}
    \end{tabular}
    \caption{\hl{Correlation between propaganda and coordination...}\label{tab:corr-prop-vs-coord}}
\end{table}


==> unused/tab-corr-prop-vs-suspensions.tex <==
\begin{table}[t]
    \scriptsize
    \centering
    \begin{tabular}{lcrlcrl}
        \toprule
        \textbf{community} && \multicolumn{2}{c}{$r$} && \multicolumn{2}{c}{$\delta$ (\%)} \\
        \midrule
        \texttt{LAB} && $0.925$ & *** && $-0.016$ & ($-6.5\%$) \\
        \texttt{CON} && $-0.079$ &  && $-0.008$ & ($-3.0\%$) \\
        \texttt{TVT} && $0.844$ & *** && $+0.074$ & ($+26.0\%$) \\
        \texttt{SNP} && $0.902$ & *** && $-0.031$ & ($-13.5\%$) \\
        \texttt{B60} && $0.882$ & *** && $-0.070$ & ($-36.7\%$) \\
        \texttt{ASE} && $-0.218$ &  && $+0.026$ & ($+9.7\%$) \\
        \texttt{LCH} && $-0.733$ & *** && $+0.014$ & ($+20.7\%$) \\
        \midrule
        overall && $-0.052$ &  && \multicolumn{2}{c}{--} \\
        \bottomrule
        \multicolumn{7}{l}{***: $p < 0.01$, **: $p < 0.05$, *: $p < 0.1$}
    \end{tabular}
    \caption{\hl{Correlation between propaganda and suspensions...}\label{tab:corr-prop-vs-suspensions}}
\end{table}


==> unused/tab-tweet-examples.tex <==
% \usepackage{multirow}
% \usepackage{hyperref}
\begin{table*}[t]
    \scriptsize
    \centering
    \begin{tabular}{|p{0.1\linewidth}|p{0.6\linewidth}|p{0.3\linewidth}|}
        \toprule
        Community & Tweet Text & Article Title\\[0.5ex] 
        \midrule
        \multirow{}TVT & Join @fckboris \& \#RegisterToVote \#GE2019 & Five ways to say Fck Boris \\[0.5ex] \cline{2-3} 
        & GE2019: Five ways to say F**k Boris \#GeneralElection2019\#Brexit\#VoteToriesOut \url{http://newsnow.co.uk/share?u=https%3A//www.redpepper.org.uk/five-ways-to-say-fck-boris/&sgt=shv2&sg=cf81420b&sid=2}  & Five ways to say Fck Boris  \\[0.5ex] \cline{2-3} 
        & KARMA: Katie Hopkins forced to sell £1m home and now rents after cringe libel loss / \#GE2019 \#Brexit \url{https://mirror.co.uk/3am/celebrity-news/katie-hopkins-forced-sell-1m-20899416?utm_source=twitter.com&utm_medium=social&utm_campaign=sharebar} & Katie Hopkins forced to sell £1m home and now rents after humiliating libel case \\[0.5ex] \cline{2-3} 
        & Here is vocal \#RemainerNow and life long Tory voter @OborneTweets on \#GE2019 \url{https://opendemocracy.net/en/opendemocracyuk/as-a-lifelong-conservative-heres-why-i-cant-vote-for-boris-johnson/} & As a lifelong Conservative, here’s why I can’t vote for Boris Johnson \\[0.5ex] \cline{2-3} 
        & Boris Johnson unfit to be Prime Minister. Brexit damages the Henley constituency -  John Howell MP knows this but continues his support-  @LauracoyleLD Laura Coyle the People’s Vote recommendation \#TacticalVoting \#PeoplesVote #Boris \#GeneralElection2019 & I was Boris Johnson’s boss: he is utterly unfit to be prime minister \\[0.5ex] \cline{2-3} 
        & This is beyond desperate and beyond tin pot banana republic actions if true. \#GE2019 & General election: Farage claims No 10 offered Brexit Party candidates jobs to stand down \\[0.5ex]
        \hline
        \multirow{}B60 & I’m voting Labour for the final say on Brexit. Share why you’re voting Labour Right \#VoteLabour \url{http://labour.org.uk/votinglabour?utm_campaign=ge19_votinglabour&utm_source=bsd&utm_medium=website&source=20191210_ge19_votinglabour&subsource=bsd_website} & I'm Voting Labour… \\[0.5ex] \cline{2-3} 
        & I’m voting Labour for a million green jobs. Share why you’re voting Labour \#VoteLabour  \url{http://labour.org.uk/votinglabour?utm_campaign=ge19_votinglabour&utm_source=bsd&utm_medium=website&source=20191210_ge19_votinglabour&subsource=bsd_website}  & I'm Voting Labour…  \\[0.5ex] \cline{2-3}
        & WASPI Women won’t be silenced \#GeneralElection2019 \url{https://waspi.co.uk/2019/11/08/waspi-women-wont-be-silenced-generalelection2019/} via @WASPI\_Campaign & WASPI Women won’t be silenced \#GeneralElection2019 \\[0.5ex] \cline{2-3}
        & Owen Jones: ‘They don’t want you to vote. Defy them’ \#GTTO  \#GeneralElection2019 \url{https://f7td5.app.goo.gl/GZYmbz} Sent via @updayUK & Owen Jones: ‘They don’t want you to vote. Defy them’  \\[0.5ex] \cline{2-3} 
        & Deadline is tomorrow! \#RegisterToVote \#vote \#ge2019 \url{https://gov.uk/register-to-vote} & Register to vote \\[0.5ex] \cline{2-3} 
        & You need to register to vote before 23:59 TONIGHT! GET. ON. IT. \url{http://bit.ly/2KSpaPy} \#GE2019 & Register to vote \\[0.5ex] \cline{2-3} 
        & Well done May from Falkirk Waspi. \url{https://gloucestershirelive.co.uk/news/cheltenham-news/waspi-woman-puts-boris-johnson-3570246?fbclid=IwAR15TmdpApchnJ3FXng4G0JVC4OXR7Y6cJ70JdLU28UJ6VpnPAo7aMavS1Q} \#waspicampaign2018 \#deedsnotwords \#onevoice \#GeneralElection2019 & WASPI woman puts Boris Johnson on spot about trust after he publicly pledged to try and sort out pension row during visit to Cheltenham \\[0.5ex] \cline{2-3}
        & Now that most party manifestos have been published, join  @WASPI\_Campaign today at \url{http://waspi.co.uk/how-to-join/} and find your nearest local group at \url{http://waspi.co.uk/find-a-local-group/} to find out about our \#GE2019 Toolkit so you can speak up for \#WASPI in your local area \#WASPIwomenvote & How to join WASPI \\[0.5ex] 
        \bottomrule
    \end{tabular}
\caption{Short summary of the activity for the most coordinated (coordination $\geq$ 0.9) members of two opposite communities. Tweets for TVT are ones flagged by \texttt{Proppy} as
propaganda, and for B60 - not propaganda. In terms of article/URL shares, these are some of the most frequent.}\label{tab:tweet-examples}
\end{table*}

